Intensity-Free Learning of Temporal Point Processes

Temporal point processes are the dominant paradigm for modeling sequences of events happening at irregular intervals. The standard way of learning in such models is by estimating the conditional intensity function. However, parameterizing the intensity function usually incurs several trade-offs. We show how to overcome the limitations of intensity-based approaches by directly modeling the conditional distribution of inter-event times. We draw on the literature on normalizing flows to design models that are flexible and efficient. We additionally propose a simple mixture model that matches the flexibility of flow-based models, but also permits sampling and computing moments in closed form. The proposed models achieve state-of-the-art performance in standard prediction tasks and are suitable for novel applications, such as learning sequence embeddings and imputing missing data.

==> tables/data_description.tex <==
\begin{tabular}{lrrr}
\toprule
    Dataset name &  Number of sequences &  Number of classes &  Total number of events \\
\midrule
          Lastfm &                  929 &               3150 &                 1268385 \\
     Memetracker &                   50 &                  1 &                  223480 \\
          Mimic2 &                  650 &                 75 &                    2419 \\
            Mooc &                 7047 &                 97 &                  396633 \\
          Reddit &                10000 &                984 &                  672350 \\
  Stack overflow &                 6633 &                 22 &                  480414 \\
       Wikipedia &                 1000 &               8227 &                  157471 \\
         Hawkes1 &                   64 &                  1 &                   65536 \\
         Hawkes2 &                   64 &                  1 &                   65536 \\
         Poisson &                   64 &                  1 &                   65536 \\
         Renewal &                   64 &                  1 &                   65536 \\
 Self correcting &                   64 &                  1 &                   65536 \\
\bottomrule
\end{tabular}


==> tables/mark_results.tex <==
\begin{tabular}{lrrrrrr}
\toprule
Model & \multicolumn{3}{l}{\$p(x | t)\$} & \multicolumn{3}{l}{\$p(x)\$} \\
RNN type &        GRU &   LSTM &    RNN &    GRU &   LSTM &    RNN \\
Dataset        &            &        &        &        &        &        \\
\midrule
Mimic2         &      1.426 &  1.449 &  1.419 &  1.423 &  1.441 &  1.431 \\
Stack overflow &      2.005 &  2.010 &  2.038 &  2.023 &  2.030 &  2.055 \\
\bottomrule
\end{tabular}


==> tables/mark_results_final.tex <==
\begin{tabular}{lrrrrrr}
    \toprule
    & \multicolumn{3}{l}{$p(\Mark | \DeltaTime)$} & \multicolumn{3}{l}{$p(\Mark)$} \\
    &                       GRU &   LSTM &    RNN &    GRU &   LSTM &    RNN \\
    \midrule
    Mimic2         &\textbf{1.426} &  1.449 &  1.419 &  1.423 &  1.441 &  1.431 \\
    Stack overflow &\textbf{2.005} &  2.010 &  2.038 &  2.023 &  2.030 &  2.055 \\
    \bottomrule
\end{tabular}


==> tables/marks_accuracy_results.tex <==
\begin{tabular}{lcc}
\toprule
{} &          Reddit &            MOOC \\
\midrule
LogNormMix &  0.62$\pm$0.013 &  0.42$\pm$0.005 \\
DSFlow     &  0.62$\pm$0.013 &  0.45$\pm$0.004 \\
SOSFlow    &  0.62$\pm$0.013 &  0.46$\pm$0.009 \\
FullyNN    &  0.63$\pm$0.013 &  0.46$\pm$0.004 \\
LogNormal  &  0.62$\pm$0.014 &  0.45$\pm$0.003 \\
RMTPP      &  0.62$\pm$0.014 &  0.41$\pm$0.006 \\
\bottomrule
\end{tabular}


==> tables/marks_mark_nll_results.tex <==
\begin{tabular}{lcc}
\toprule
{} &          Reddit &            MOOC \\
\midrule
LogNormMix &  2.12$\pm$0.113 &  1.83$\pm$0.016 \\
DSFlow     &  2.11$\pm$0.090 &  1.74$\pm$0.013 \\
SOSFlow    &  2.14$\pm$0.110 &  1.72$\pm$0.024 \\
FullyNN    &  2.10$\pm$0.115 &  1.71$\pm$0.010 \\
LogNormal  &  2.09$\pm$0.094 &  1.73$\pm$0.009 \\
RMTPP      &  2.11$\pm$0.104 &  1.85$\pm$0.023 \\
\bottomrule
\end{tabular}


==> tables/marks_nll_results.tex <==
\begin{tabular}{lcc}
\toprule
{} &           Reddit &             MOOC \\
\midrule
LogNormMix &  12.40$\pm$0.094 &   7.58$\pm$0.047 \\
DSFlow     &  12.39$\pm$0.064 &   7.52$\pm$0.074 \\
SOSFlow    &  12.49$\pm$0.158 &   7.78$\pm$0.107 \\
FullyNN    &  12.51$\pm$0.094 &   7.93$\pm$0.230 \\
LogNormal  &  12.51$\pm$0.080 &   8.11$\pm$0.026 \\
RMTPP      &  13.26$\pm$0.085 &  12.14$\pm$0.220 \\
\bottomrule
\end{tabular}


==> tables/marks_time_nll_results.tex <==
\begin{tabular}{lcc}
\toprule
{} &           Reddit &             MOOC \\
\midrule
LogNormMix &  10.28$\pm$0.066 &   5.75$\pm$0.040 \\
DSFlow     &  10.28$\pm$0.073 &   5.78$\pm$0.067 \\
SOSFlow    &  10.35$\pm$0.106 &   6.06$\pm$0.084 \\
FullyNN    &  10.41$\pm$0.079 &   6.22$\pm$0.224 \\
LogNormal  &  10.42$\pm$0.076 &   6.38$\pm$0.019 \\
RMTPP      &  11.15$\pm$0.061 &  10.29$\pm$0.209 \\
\bottomrule
\end{tabular}


==> tables/results_with_history.tex <==
\begin{tabular}{lrrrrrrrrr}
\toprule
Model &   CDF  &  CDF Hyper &  CDF Residual &  Flow MLP &  Flow Sin &  Flow Softplus &  FullyNN &  Mixture &  RMTPP \\
Dataset         &        &            &               &           &           &                &          &          &        \\
\midrule
Hawkes1         & -0.394 &     -0.393 &        -0.395 &    -0.261 &    -0.394 &         -0.369 &   -0.363 &   -0.394 & -0.332 \\
Hawkes2         & -0.966 &     -0.963 &        -0.965 &    -0.836 &    -0.960 &         -0.947 &   -0.912 &   -0.966 & -0.575 \\
Lastfm          & -4.560 &     -4.564 &        -4.559 &    -4.190 &    -4.525 &         -4.514 &   -4.390 &   -4.543 & -3.447 \\
Memetracker     & -1.915 &     -1.877 &        -1.911 &    -1.531 &    -1.850 &         -1.789 &   -1.755 &   -1.894 & -1.700 \\
Mimic2          &  0.501 &      0.496 &         0.498 &     0.548 &     0.516 &          0.504 &    0.543 &    0.495 &  0.598 \\
Mooc            & -5.690 &     -5.474 &        -5.635 &    -5.036 &    -5.265 &         -5.289 &   -4.603 &   -5.497 & -2.346 \\
Poisson         &  1.003 &      1.002 &         1.003 &     1.058 &     1.003 &          1.032 &    1.017 &    1.001 &  1.000 \\
Reddit          & -1.056 &     -1.034 &        -1.055 &    -0.578 &    -1.010 &         -0.993 &   -0.959 &   -1.022 & -0.385 \\
Renewal         & -1.211 &     -1.212 &        -1.212 &    -1.199 &    -1.212 &         -1.212 &   -1.164 &   -1.208 & -0.919 \\
Self correcting &  1.106 &      1.109 &         1.106 &     1.378 &     1.115 &          1.146 &    1.115 &    1.106 &  1.102 \\
Stack overflow  &  0.562 &      0.563 &         0.562 &     0.714 &     0.561 &          0.564 &    0.609 &    0.568 &  0.627 \\
Wikipedia       & -2.378 &     -2.380 &        -2.377 &    -2.156 &    -2.378 &         -2.373 &   -2.271 &   -2.372 & -1.378 \\
\bottomrule
\end{tabular}


==> tables/results_without_history.tex <==
\begin{tabular}{lrrrrrrrrr}
\toprule
Model &   CDF  &  CDF Hyper &  CDF Residual &  Flow MLP &  Flow Sin &  Flow Softplus &  FullyNN &  Mixture &  RMTPP \\
Dataset         &        &            &               &           &           &                &          &          &        \\
\midrule
Hawkes1         & -0.267 &     -0.266 &        -0.265 &    -0.261 &    -0.252 &         -0.243 &   -0.247 &   -0.268 & -0.150 \\
Hawkes2         & -0.876 &     -0.877 &        -0.874 &    -0.837 &    -0.857 &         -0.852 &   -0.836 &   -0.859 & -0.386 \\
Lastfm          & -4.219 &     -4.220 &        -4.220 &    -4.197 &    -4.163 &         -4.104 &   -4.014 &   -4.223 & -2.647 \\
Memetracker     & -1.622 &     -1.616 &        -1.620 &    -1.531 &    -1.540 &         -1.527 &   -1.458 &   -1.527 & -1.206 \\
Mimic2          &  0.478 &      0.479 &         0.477 &     0.547 &     0.499 &          0.497 &    0.492 &    0.484 &  0.577 \\
Mooc            & -5.725 &     -5.908 &        -5.562 &    -5.069 &    -5.079 &         -5.039 &   -4.599 &   -5.066 & -2.252 \\
Poisson         &  1.005 &      1.006 &         1.005 &     1.057 &     1.030 &          1.097 &    1.016 &    1.003 &  1.000 \\
Reddit          & -0.635 &     -0.635 &        -0.629 &    -0.579 &    -0.609 &         -0.580 &   -0.575 &   -0.621 & -0.054 \\
Renewal         & -1.208 &     -1.207 &        -1.207 &    -1.198 &    -1.203 &         -1.203 &   -1.170 &   -1.188 & -0.922 \\
Self correcting &  1.259 &      1.260 &         1.261 &     1.378 &     1.284 &          1.388 &    1.267 &    1.261 &  1.267 \\
Stack overflow  &  0.682 &      0.682 &         0.682 &     0.714 &     0.683 &          0.760 &    0.716 &    0.683 &  0.725 \\
Wikipedia       & -2.168 &     -2.165 &        -2.167 &    -2.156 &    -2.167 &         -2.163 &   -2.083 &   -2.168 & -1.073 \\
\bottomrule
\end{tabular}


==> tables/test_nll_results.tex <==
\begin{tabular}{lcccccc}
\toprule
{} &             Yelp &           Reddit &           LastFM &             MOOC &   Stack Overflow &        Wikipedia \\
\midrule
LogNormMix &  13.02$\pm$0.070 &  10.19$\pm$0.078 &  -2.88$\pm$0.147 &   6.03$\pm$0.092 &  14.44$\pm$0.013 &   8.39$\pm$0.079 \\
DSFlow     &  13.09$\pm$0.065 &  10.20$\pm$0.074 &  -2.88$\pm$0.148 &   6.03$\pm$0.090 &  14.44$\pm$0.019 &   8.40$\pm$0.090 \\
SOSFlow    &  13.21$\pm$0.068 &  10.27$\pm$0.106 &  -2.56$\pm$0.133 &   6.27$\pm$0.058 &  14.47$\pm$0.049 &   8.44$\pm$0.120 \\
FullyNN    &  13.04$\pm$0.073 &  10.23$\pm$0.072 &  -2.84$\pm$0.179 &   6.83$\pm$0.152 &  14.45$\pm$0.014 &   8.40$\pm$0.086 \\
LogNormal  &  13.44$\pm$0.074 &  10.38$\pm$0.077 &  -2.60$\pm$0.140 &   6.53$\pm$0.016 &  14.62$\pm$0.013 &   8.52$\pm$0.078 \\
RMTPP      &  13.36$\pm$0.056 &  10.88$\pm$0.293 &  -1.30$\pm$0.164 &  10.65$\pm$0.023 &  14.51$\pm$0.014 &  10.02$\pm$0.085 \\
\bottomrule
\end{tabular}


==> tables/test_nll_results_synth.tex <==
\begin{tabular}{lccccc}
\toprule
{} &         Poisson &         Renewal & Self-correcting &         Hawkes1 &         Hawkes2 \\
\midrule
LogNormMix &  0.99$\pm$0.006 &  0.25$\pm$0.010 &  0.78$\pm$0.003 &  0.52$\pm$0.047 &  0.02$\pm$0.049 \\
DSFlow     &  0.99$\pm$0.006 &  0.25$\pm$0.010 &  0.78$\pm$0.002 &  0.52$\pm$0.047 &  0.02$\pm$0.050 \\
SOSFlow    &  1.00$\pm$0.013 &  0.25$\pm$0.010 &  0.88$\pm$0.011 &  0.59$\pm$0.056 &  0.06$\pm$0.046 \\
FullyNN    &  1.00$\pm$0.006 &  0.28$\pm$0.013 &  0.78$\pm$0.004 &  0.55$\pm$0.047 &  0.06$\pm$0.047 \\
LogNormal  &  1.08$\pm$0.008 &  0.25$\pm$0.010 &  1.03$\pm$0.006 &  0.55$\pm$0.047 &  0.06$\pm$0.049 \\
RMTPP      &  0.99$\pm$0.006 &  1.01$\pm$0.023 &  0.78$\pm$0.003 &  0.74$\pm$0.057 &  0.69$\pm$0.058 \\
\bottomrule
\end{tabular}

